State-dependent Riccati equation feedback stabilization for nonlinear PDEs

The synthesis of suboptimal feedback laws for controlling nonlinear dynamics arising from semi-discretized PDEs is studied. An approach based on the State-dependent Riccati Equation (SDRE) is presented for H2 and Hinf control problems. Depending on the nonlinearity and the dimension of the resulting problem, offline, online, and hybrid offline-online alternatives to the SDRE synthesis are proposed. The hybrid offline-online SDRE method reduces to the sequential solution of Lyapunov equations, effectively enabling the computation of suboptimal feedback controls for two-dimensional PDEs. Numerical tests for the Sine-Gordon, degenerate Zeldovich, and viscous Burgers' PDEs are presented, providing a thorough experimental assessment of the proposed methodology.

==> nla.tex <==
%\documentclass{siamart171218}
%
%\usepackage{amsmath,amssymb,amsfonts,color}
%\usepackage{algorithmic}
%%\usepackage{algorithm,booktabs}
%%\usepackage[mathscr]{eucal}
%\usepackage{graphicx}
%\usepackage{todonotes}
%\usepackage{epstopdf}
%%\usepackage{mathdots} % use [H] in figure environments
%\usepackage{showlabels}
%\usepackage{graphics}
%
%\newcommand{\RR}{\mathbb{R}}
%\newcommand{\ale}[2][red]{\emph{\textcolor{#1}{#2}}}
%\newcommand{\dante}[2][blue]{\emph{\textcolor{#1}{#2}}}
%\newcommand{\vale}[2][cyan]{\emph{\textcolor{#1}{#2}}}
%
%\newcommand{\cA}{\mathcal{A}}
%\newcommand{\cC}{\mathcal{C}}
%\newcommand{\cF}{\mathcal{F}}
%\newcommand{\R}{\mathbb{R}}
%\newcommand{\bD}{\mathbb{D}}
%\newcommand{\cI}{\mathcal{I}}
%\newcommand{\cG}{\mathcal{G}}
%\newcommand{\cM}{\mathcal{M}}
%\newcommand{\cO}{\mathcal{O}}
%\newcommand{\cP}{\mathcal{P}}
%\newcommand{\cQ}{\mathcal{Q}}
%\newcommand{\cU}{\mathcal{U}}
%\newcommand{\cV}{\mathcal{V}}
%\newcommand{\cN}{\mathcal{N}}
%\newcommand{\cJ}{\mathcal{J}}
%\newcommand{\lt}{\left}
%\newcommand{\rt}{\right}
%
%
%\begin{document}


\section{Solving large-scale Algebraic Riccati/Lyapunov equations}

The time steps discussed in Section~\ref{secsdre} all use 
matrices that stem from the solution of algebraic matrix equations,
and more precisely the (quadratic) Riccati and the (linear) Lyapunov equations. 
The past few years have seen
a dramatic improvement in the effectiveness of numerical solution strategies
for solving these equations in the large scale setting. For a survey
in the linear case we refer the reader to the recent article \cite{Simoncini.survey.16}, while
for the algebraic Riccati equation we point 
the reader to, e.g., \cite{B08,SSM14,Binietal.book.12}.

%Some of the developed approaches adapt particularly well to our setting. 
In our derivation we found 
projection methods to be able to adapt particularly well
to the considered setting, with a similar reduction
framework for both linear and quadratic methods, other approaches are
reviewed for instance in \cite{Benner.Saak.survey13,Simoncini.survey.16}. We emphasize that
all considered methods require that the zero order term in the matrix equation, e.g., matrix $Q$ in
the Riccati equation \eqref{sdre1}, be low rank.

The general idea consists of first determining an approximation space ${\cal K}_k$ that can be naturally
expanded if needed, and then seeking an approximate solution in this space, by imposing a Galerkin condition on the matrix residual for computing the projected approximate solution.

Let ${\cal V}_k$ be such that ${\cal K}_k={\rm range}({\cal V}_k)$, with ${\cal V}_k$ having orthonormal columns. Recalling that in both
the Riccati and Lyapunov equations the solution matrix is symmetric, the approximate
solution can be written as  ${\cal V}_k Y {\cal V}_k^\top$. 

Consider the Riccati equation \eqref{sdre1} for a fixed $x=x(t_*)$, so that we set $A(x(t_*))=A_*$ and
$B(x(t_*))=B_*$. 
Let ${\cal R} = A_*^\top {\cal V}_k Y_X {\cal V}_k^\top + {\cal V}_k Y_X {\cal V}_k^\top A_* -
{\cal V}_k Y_X {\cal V}_k^\top B_* {\cal V}_k Y_X {\cal V}_k^\top + Q$.
Imposing the Galerkin condition on ${\cal R}$ means that the residual matrix ${\cal R}$ be orthogonal to 
the approximation space, in the matrix sense, that is
\begin{equation}\label{eqn:reduced_Riccati}
{\cal V}_k^\top {\cal R} {\cal V}_k =0 \quad 
\Leftrightarrow \quad
{\cal V}_k^\top A_*^\top {\cal V}_k Y_X +  Y_X {\cal V}_k^\top A_* {\cal V}_k -
 Y_X ({\cal V}_k^\top B_* {\cal V}_k) Y_X  + {\cal V}_k^\top Q {\cal V}_k=0,
\end{equation}
where the orthogonality of the columns of ${\cal V}_k$ was used.
If ${\cal V}_k$ has small dimensions, the {\it reduced} Riccati matrix equation 
on the right also has small dimensions and can be solved by a ``dense'' method
to determine $Y_X$; see, e.g., 
\cite{Binietal.book.12}.
The cost of solving the reduced quadratic equation with coefficient matrices of size $\hat k$ 
is at least $63 \hat k^3$ floating point operations with an invariant subspace approach
\cite{Laub.79}.
Note that the large matrix ${\cal V}_k Y_X {\cal V}_k^\top$ is never
constructed explicitly, since it would be dense even for sparse data.

Analogously, for the Lyapunov equation in \eqref{lyap_on}, we can write $W \approx {\cal V}_k Y {\cal V}_k^\top$
for some $Y=Y_W$ to be determined. Let ${\cal Q}_* = \sum_k Q_k f_k(x(t_*))$. As before, letting $\widetilde{\cal R} = C_0^\top {\cal V}_k Y {\cal V}_k^\top + {\cal V}_k Y {\cal V}_k^\top C_0
+ {\cal Q}_*$, the Galerkin condition leads to
$$
{\cal V}_k^\top \widetilde{\cal R} {\cal V}_k =0 \quad \Leftrightarrow \quad
 ({\cal V}_k^\top C_0^\top {\cal V}_k) Y  + Y {\cal V}_k^\top C_0 {\cal V}_k
+ {\cal V}_k^\top{\cal Q}_* {\cal V}_k = 0.
$$
This {\it reduced} Lypaunov equation can be solved by means of a ``dense'' method at a cost
of about 15 $\hat k^3$ floating point operations for coefficient matrices of size
$\hat k$, if the real Schur decomposition is employed; see, e.g.,
\cite{Simoncini.survey.16}. Note that the computational cost is significantly lower than
that of solving the reduced Riccati equation with matrices of the same size.


\subsection{On the selection of the approximation space}
 Choices as approximation space explored in the literature
include polynomial and rational Krylov subspaces
\cite{Simoncini.survey.16}. They both enjoy the property of being nested as they enlarge, that is
${\cal K}_k \subseteq {\cal K}_{k+1}$ where $k$ is associated with the space dimension.
Rational Krylov subspaces have emerged as the key choice because they are able to deliver
accurate  approximate solutions with a relatively small space dimension, compared with polynomial
spaces. Given a starting tall matrix $V_0$ and an invertible stable coefficient matrix
$A_*$, we have used two distinct rational spaces: the Extended Krylov subspace,
$$
{\cal E}{\cal K}_k = {\rm range}([V_0, A_*^{-1} V_0, A_* V_0, A_*^{-2} V_0, A_*^2 V_0, \ldots, 
A_*^{k-1} V_0, A_*^{-k} V_0]),
$$
which only involves matrix-vector products and solves with $A_*$, and the (fully) Rational Krylov subspace,
$$
{\cal R}{\cal K}_ k =
{\rm range}([V_0, (A_*- \sigma_2 I)^{-1} V_0, \ldots, \prod_{j=2}^k (A_*- \sigma_j I)^{-1} V_0]) .
$$
where $\sigma_j$ can be computed a-priori or adaptively.
In both cases, the space is expanded iteratively, one block of vectors at the time,
and systems with $A_*$ or with $(A_*- \sigma_j I)$ are solved by fast sparse methods.

In our implementation we used the Extended Krylov subspace for solving the Lyapunov equation
in Algorithm \ref{Alg_sdreon}, which has several advantages, such as the computation of the sparse Cholesky factorization of $A_0$ once for all.
 On the other hand, we used the Rational Krylov subspace for the Riccati equation, which
has been shown to be largely superior over the Extended Krylov on this quadratic equation,
in spite of requiring the solution of a different (shifted) sparse coefficient matrix at each iteration 
\cite{Benner.Saak.survey13,SSM14}.
Nonetheless, in Section~\ref{sec:feedback_matrix} we report an alternative approach that
makes the Extended Krylov subspace competitive again for the Riccati problem with $A_0$ symmetric.
%
Except for the operations associated with the reduced problems, the computational costs per iteration of the
Riccati and Lyapunov equation solvers are very similar, if the same approximation space is used.
%Regarding the approximation space, the rational Krylov space requires solving with a different (shifted)
%sparse coefficient matrix at each iteration, and is thus more expensive than building the Extended space.
%However, experimental evidence and theoretical arguments have supported the use of the rational Krylov
%subspace in many cases \cite{Benner.Saak.survey13,SSM14,Simoncini.survey.16}.


Although we refer to the specialized literature for the algorithmic 
details\footnote{See {\tt www.dm.unibo.it/$\widetilde{\mbox{ }}$simoncin/software} for some related software.},
we would like to include some important implementation details that are specific to our
setting. 
In particular, the matrix $C_0$ employed in Algorithm \ref{Alg_sdreon} is given by
$C_0 = A_0 - \left(BR^{-1} B^\top - \frac 1 {2\gamma^2} H P^{-1} H^\top\right) \Pi_0$, which is
not easily invertible if explicitly written, since it is dense in general. Note that
$A_0$ is in general sparse, as it stems from the discretization of a partial differential
operator. We can write
%$$
%C_0 = A_0 - \left([B, H] G [B,H]^\top\right) \Pi_0, \quad {\rm with} \quad
%G = R^{-1} - \frac 1 {2\gamma^2} P^{-1} .
%$$
$$
C_0 = A_0 - \left([B, H] G [B,H]^\top\right) \Pi_0, \quad {\rm with} \quad
G = \begin{pmatrix} 
R^{-1}& 0\\
0 & - \frac 1 {2\gamma^2} P^{-1}
\end{pmatrix}.
$$
Using the classical Sherman-Morrison-Woodbury formula, the product $C_0^{-1} V$ for some
tall matrix $V$ can be obtained as 
$$
W:=C_0^{-1} V = A_0^{-1} V - A_0^{-1} [B, H] G_1^{-1} [B,H]^\top \Pi_0 A_0^{-1}V,
$$
with $G_1 = I + G [B,H]^\top \Pi_0 A_0^{-1} [B, H]$, which is assumed to be nonsingular. 
Therefore, $C_0^{-1} V$  can be obtained
by first solving sparse linear systems with $A_0$, and then using matrix-matrix products.
More precisely, the following steps are performed:

\vskip 0.1in

- Solve $A_0 W_1 = V$

- Solve $A_0 W_2 = [B, H]$

- Compute $G_1 = I + G [B,H]^\top \Pi_0 W_2$

- Compute $W = W_1 - W_2 ( \, G_1^{-1} ( [B,H]^\top \Pi_0 W_1) \, )$

\vskip 0.1in
We also recall that $\Pi_0$, the solution to the initial Riccati equation, is stored
in factored form, and this should be taken into account when computing matrix-matrix
products with $\Pi_0$.

While trying to employ the Rational Krylov space, we found that the structure of $C_0$ 
made the selection of optimal shifts $\{\sigma_j\}$ particularly challenging, resulting
in a less effective performance of the method. Hence, our preference went for
the Extended Krylov space above, with the above
enhancement associated with solves with $C_0$.


\subsection{Feedback matrix oriented implementation}\label{sec:feedback_matrix}
In Algorithm \ref{Alg_sdre} the Riccati equation needs to be solved at each
time step $t_n$. However, its solution $\Pi(x_n)$ is only used to computed the feedback matrix 
$K(x_n) : = - R^{-1} B^\top \Pi(x_n)$. Hence, it would be desirable to be able to
immediately compute $K(x_n)$ without first computing $\Pi(x_n)$. This approach
has been explored in the Riccati equation literature but also for
other problems based on Krylov 
subspaces, see, e.g., \cite{Palitta.Simoncini.18a,Kressner.proc.2008}.

In this section, in the case where the matrix $A(x_n)$ is symmetric,
 we describe the implementation of one of the projection methods described above,
that is able to directly compute $K(x_n)$ without computing $\Pi(x_n)$ (in factored form), and
more importantly, without storing and computing the whole approximation basis. 
The latter feature is particularly important for large scale problems, for which dealing
with the orthogonal approximation basis represents one of the major computational and
memory costs. To the best of our knowledge, this variant of the Riccati solver is new, while it is currently explored in \cite{Palitta.Pozza.Simoncini.21} for the rational Krylov space.

Here we consider, the Extended Krylov subspace. For $A(x_n)$ symmetric, the 
orthonormal basis of ${\cal E}{\cal K}_k$
can be constructed by explicitly orthogonalizing only with respect
to the previous two basis blocks. Hence, only two previous blocks of vectors need to
be stored in memory, and require explicitly orthogonalization when the new block of vectors
is added to the basis \cite{Palitta.Simoncini.18a}. This is also typical of polynomial
Krylov subspaces costructed for symmetric matrices, giving rise to the classical Lanczos three-term recurrence \cite{Kressner.proc.2008}. 
%We also refer to the recent manuscript \cite{Palitta.Pozza.Simoncini.21} for a similar derivation when using the rational Krylov subspace.

With this procedure, in the reduced equation \eqref{eqn:reduced_Riccati} 
the matrices $A_k := {\cal V}_k^\top A_* {\cal V}_k$, 
$B_k := {\cal V}_k^\top B$ and $Q_k:={\cal V}_k^\top Q {\cal V}_k$
are computed as $k$ grows by updating the new terms at each iteration, and
the solution $Y_X$ can be obtained without the whole matrix ${\cal V}_k$ being available.
Note that the stopping criterion does not require the computation of the whole residual
matrix, so that also in the standard solver
the matrix ${\cal V}_k Y_X {\cal V}_k^\top$ is never required until completion.

However, to be able to compute 
$$
K = -R B^\top {\cal V}_k Y_X {\cal V}_k^\top = -R B_k^\top Y_X {\cal V}_k^\top,
$$
the basis ${\cal V}_k$ appearing on the right still seems to be required.
As already done in the literature, this problem can be overcome by a so-called ``two-step'' 
procedure: at completion, once the final $Y_X$ is available,
 the basis ${\cal V}_k$ is computed again one block at the
time, and the corrisponding terms in the product $Y_X {\cal V}_k^\top$ are updated.
Since $A(x_n)$ is already factorized and the orthogonalization coefficients are already
available (they correspond to the nonzero entries of $A_k$), then the overall computational
cost is accessible; we refer the reader to \cite{Palitta.Simoncini.18a} and its references
for additional details for the two-step procedure employed for different purposes.



%\end{document}
%
%{
%@Article{Simoncini.survey.16,
%  author    = {V.~Simoncini},
%  journal   = {SIAM Rev.},
%  title     = {Computational methods for linear matrix equations},
%  year      = {2016},
%  month     = {Sept},
%  number    = {3},
%  pages     = {377-441},
%  volume    = {58},
%  file      = {:/home/valeria/Bibl/Papers/sirev58-3_377.pdf:PDF},
%  owner     = {valeria},
%  timestamp = {2013.07.01},
%}
%
%@Article{Palitta.Simoncini.18a,
%  author    = {D. Palitta and V. Simoncini},
%  journal   = {J. Comput. Applied Math.},
%  title     = {Computationally enhanced projection methods for symmetric Sylvester and Lyapunov matrix equations},
%  year      = {2018}, pages={648--659},
%  volume    = {330},
%  owner     = {valeria},
%  timestamp = {2018.04.17},
%}
%@Article{Palitta.Simoncini.18b,
%  author    = {D. Palitta and V. Simoncini},
%  journal   = {SIAM J. Sci. Comput},
%  title     = {Numerical methods for large-scale {L}yapunov equations with symmetric banded data},
%  year      = {2018},
%  number    = {5},
%  volume    = {40},
%  file      = {:/home/valeria/Bibl/Papers/17m1156575.pdf:PDF},
%  mynote    = {arXiv 1711.04187},
%  owner     = {valeria},
%  timestamp = {2018.04.17},
%}
%
%@Book{Binietal.book.12,
%  Title                    = {Numerical Solution of Algebraic Riccati Equations},
%  Author                   = {D.A. Bini and B. Iannazzo and B. Meini},
%  Publisher                = {SIAM},
%  Year                     = {2012},
%
%  Address                  = {Philadelphia},
%
%  Bookseries               = {Book Series Fundamentals of Algorithms},
%  Owner                    = {valeria},
%  Timestamp                = {2012.02.09}
%}
%
%@TechReport{Palitta.Pozza.Simoncini.21,
%  author    = {D. Palitta and S. Pozza and V. Simoncini},
%  number   = {arXiv:2103.04054 },
%  title     = {The short-term rational Lanczos method and applications},
%  year      = {2018},
%  institution    = {arXiv}
%}
%
%%%}

